Multi-grained Semantics-aware Graph Neural Networks

Graph Neural Networks (GNNs) are powerful techniques in representation learning for graphs and have been increasingly deployed in a multitude of different applications that involve node- and graph-wise tasks. Most existing studies solve either the node-wise task or the graph-wise task independently while they are inherently correlated. This work proposes a unified model, AdamGNN, to interactively learn node and graph representations in a mutual-optimisation manner. Compared with existing GNN models and graph pooling methods, AdamGNN enhances the node representation with the learned multi-grained semantics and avoids losing node features and graph structure information during pooling. Specifically, a differentiable pooling operator is proposed to adaptively generate a multi-grained structure that involves meso- and macro-level semantic information in the graph. We also devise the unpooling operator and the flyback aggregator in AdamGNN to better leverage the multi-grained semantics to enhance node representations. The updated node representations can further adjust the graph representation in the next iteration. Experiments on 14 real-world graph datasets show that AdamGNN can significantly outperform 17 competing models on both node- and graph-wise tasks. The ablation studies confirm the effectiveness of AdamGNN's components, and the last empirical analysis further reveals the ingenious ability of AdamGNN in capturing long-range interactions.

==> pages/cover_letter.tex <==
\onecolumn
\section{Cover Letter}
Dear Editors:

We submit hereby the manuscript entitled ``Multi-grained Semantics-aware Graph Neural Networks”, which we wish to be considered for publication in IEEE Transactions on Knowledge and Data Engineering. 
No conflict of interest exists in the submission of this manuscript, and the manuscript is approved by all authors for publication. 
I would like to declare on behalf of my co-authors that the work described was original research that has not been published previously and is not under consideration for publication elsewhere, in whole or in part. 
All the authors listed have approved the manuscript that is enclosed. We submit this manuscript based on the following reasons:

Graphs are a ubiquitous data structure, and learning representations from large graphs have been proved as a useful approach for a wide variety of graph-related tasks. 
Graph Neural Networks (GNNs) have recently attracted attention from industry and academia due to their significant performance on graph representation learning tasks. 
However, most existing studies independently solve either the node-wise task or the graph-wise task while they are inherently correlated. 
And existing graph pooling methods are significantly affected by several hyper-parameters, which reduces their convenience in applications with different scale graphs. 

To address the limitations mentioned above, we propose a novel GNN framework, Adaptive Multi-grained Graph Neural Networks (AdamGNN), which 
integrates multi-grained semantics into node representations and achieves mutual optimisation between node-wise and graph-wise tasks in one unified process.
Specifically, an adaptive and efficient pooling operator is devised in AdamGNN to generate the multi-grained structure without introducing any hyper-parameters. 
And an attention-based flyback aggregation can provide model explainability on how different grains benefit the prediction tasks.

In addition, extensive experiments conducted on $14$ real-world datasets exhibit the outstanding performance of AdamGNN in network analysis tasks, including node classification, link prediction and graph classification.
The following ablation studies confirm the effectiveness of the components of AdamGNN.
And the last model empirical analysis further reveals AdamGNN's ingenious ability in capturing long-range interactions. 

We would be very grateful if the submitted manuscript could be reviewed and considered for publication in IEEE Transactions on Knowledge and Data Engineering. We thank you in advance for handling our manuscript.


\bigskip\noindent
With best regards,

\smallskip\noindent
Yours sincerely, \\

\smallskip\noindent
Corresponding author: \\
Name: Jun Pang \\
E-mail: jun.pang@uni.lu

==> pages/response_letter.tex <==
\onecolumn
\section{Response Letter}
Dear Reviewers and Editors,

\smallskip
Thank you for giving us the opportunity to submit a revised draft of our manuscript titled ``Multi-grained Semantics-aware Graph Neural Networks” to IEEE Transactions on Knowledge and Data Engineering. 
We appreciate the time and efforts you and the reviewers have dedicated to providing your valuable feedback on our manuscript. 
We are grateful to the reviewers for their insightful comments and suggestions on our paper which helped us find shortcomings of our manuscript in terms of model design and paper writing. 
We have been able to incorporate changes to reflect most of the suggestions provided by the reviewers. 
Below is a point-by-point response to the reviewers’ comments and concerns.


\smallskip\noindent
\textbf{Comments from Reviewer 1}

\smallskip\noindent
\textbf{1.} ``The paper is titled with "semantic-aware". However, the contents of the paper including the proposed algorithm seem not so much related to "semantic-aware".''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the insightful comment, we have polished the second and third paragraphs of Section~1 to better explain the semantic information that we focused on in this paper. We present how we design the multi-grained semantic-aware GNN model in the fifth paragraph of Section 1. 
Moreover, we highlighted the ``semantic-aware'' story in Section 3. 
% 
This paper describes the relationship between nodes presented in the topology structure as semantic. 
For instance, the micro semantics is shown in the observed topological structure (e.g., co-authorship) between authors in a citation network. 
Following this way, the macro semantics refers to the relationship between different author groups, i.e., research areas or institutes (the second paragraph of Section~1).
And author groups can be naturally defined by pooling authors together (the third paragraph of Section~1). 
Therefore, we introduce the adaptive graph pooling operators to find super nodes and reveal the semantic information of different granularity levels (the fifth paragraph of Section 1). 
}

\smallskip\noindent
\textbf{2.} ``In Section 3.2 (Supernode determination section), formulation (2) is not well motivated. What are these two functions? Why do we need them? What does the probability modeled by the first function mean? For the second function, what is the "linearity relation"? Why do we need to model it for this task?''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for noticing this, we have revised the first three paragraphs of Section 3.2 to better motivate the design of Eq.~2. 
In addition, the name of $\phi_i$ we used before, i.e., the fitness score, may confuse readers, so we renamed it as the closeness score. 
% 
Particularly, the key idea of AdamGNN is applying an adaptive graph pooling operator to present the multi-grained semantics of $\mathcal{G}$ explicitly, and utilising the graph unpooling to distribute the derived meso/macro information to improve the node representation generation (the first paragraph of Section~3.2).
% 
For a graph with $n$ nodes, we can obtain $n$ ego-networks $c_{\lambda}(v_i)$ following the ego-network formulation approach (the second paragraph of Section~3.2).
Next, in the third paragraph of Section~3.2, we present how to determine which group of ego-networks should be selected as super nodes to construct the super graph, based on the closeness score $\phi_{i}$ that evaluates the representativeness of an ego $v_i$ to its local neighbours. 
Eq.~2 was designed to calculate the closeness scores, including two components to describe the similarity from non-linear and linear aspects.
That said, we performed linear and non-linear computations to calculate the closeness of an ego $v_i$ to its local neighbours, which provides a more comprehensive angle for closeness evaluation than only considering linearity or non-linearity. 
}

\smallskip\noindent
\textbf{3.} ``In Section 3.4, in Eq.~(7), why is $H_0$ separated from the other level of representations? Also, why the attention is modeled based on $H_0$.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your insightful comment, and we agree that we did not give a clear explanation about the design of Eq.~7. 
We have revised Section 3.4 to highlight the motivation of the design of Eq.~7.
% 
Specifically, the graph unpooling operator distributes the generated multi-grained semantics to the nodes in the original graph.
However, a challenging issue is how each node utilises the received semantic information with its $flat$ representation (Section 3.4). 
As the empirical exploration results that we showed in Section 4.3 (Messages from different levels.), representing nodes may need different granularity levels' information. 
Therefore, we propose to allow each node to decide whether/how to utilise semantic information from different granularity levels with an attention-enhanced mechanism. 
So, for the semantic message ($\hat{\mathbf{H}}_t$) from granularity level ($t$), we design the attention score between $\mathbf{H}$ and $\hat{\mathbf{H}}_t$ as Eq.~7 (Section 3.4). 
Therefore, $\mathbf{H}$ is separated from the other levels of representations because $\mathbf{H}$ is the primary node representation that is learned by \textit{flat} primary GNN encoder; hence it's different from other levels of representations.
Moreover, we want to utilise the multi-grained semantic representations to improve primary node representations ($\mathbf{H}$); thus, the attention is modelled based on $\mathbf{H}$ to find out which granularity level's information is more useful. 
% \CL{(need to echo to the question: why $H_0$ is separated ... why the attention is modeled based on $H_0$)}
}

\smallskip\noindent
\textbf{4.} ``In Section 3.5, How and why the reconstruction loss can alleviate the over-smoothing issue?''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the insightful comment, and we revised the second paragraph of Section~3.5 to clarify how the reconstruction loss can alleviate the over-smoothing issue. 
% 
The over-smoothing issue means nodes of a graph tend to have indistinguishable representations.
The graph reconstruction loss ($\mathcal{L}_{\it R}$) encourages disconnected nodes to have different representations to maintain the graph structure; hence it can alleviate the over-smoothing issue.
And we also verified the effectiveness of $\mathcal{L}_{\it R}$ in the ablation study of Section~4.2 (Table 7). 
% \JP{Similarly, we can add a sentence to incorporate the above explanation.}
}

\smallskip\noindent
\textbf{5.} ``In Table 4, the reported results for GCN, GAT on Cora, Citeseer, and Pubmed datasets are much lower than publicly reported results (the authors mentioned they follow the setting in GCN). This makes the reported results in this paper questionable. ''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the comment, and we agree our descriptions of ``Evaluation settings'' were not precise enough. 
We have revised the ``Evaluation settings'' of Section~4.1 to specify that we ``randomly assign $20$ labelled nodes for each class for training, and $500$ and $1000$ nodes for validation and testing, respectively.'' 
% 
Particularly, the GCN paper [3] adopts a fixed split which means they fixed a group of train/valid/test splits for experiments. 
We follow a similar approach to split train/valid/test datasets for experiments. 
But since other datasets do not have fixed splits, we ``randomly'' generated $10$ splits for experiments instead of one fixed split.
Therefore, the experimental results might slightly vary. 
Moreover, it should be noted that AdamGNN endows the \textit{flat} GNN with multi-grained semantics. Hence, it is theoretically helpful for any \textit{flat} GNN encoder, as shown in the ablation study of Section~4.3 (Ablation study of different primary GNN encoders, Table 10). 
}

\smallskip\noindent
\textbf{6.}``Furthermore, more ablation studies are needed to demonstrate the effectiveness of each component. For example, how does the multi-grained pooling process help the node classification task?''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for the concrete suggestion. Following your suggestions, 
we revised the experimental analysis sections (Sections~4.2 and 4.3) and added more ablation studies to demonstrate the effectiveness of each component of AdamGNN (Tables~7, 8, 9, 10 and Figure 3). 
% 
For the ablation study that examines the influence of different primary GNN encoders (Table 10), we find that AdamGNN can improve the performance of different GNN encoders. 
It demonstrates the effectiveness of multi-grained semantics obtained by the multi-grained pooling and unpooling process.
% 
Moreover, for the ablation studies in Section~4.2, we empirically verified the effectiveness of different loss functions (Table~7), the influence of the number of granularity levels (Table~9), the impact of Ego-network size, and the influence of different primary GNN encoders (Figure~3). 
Briefly, we found that \textit{(i)} each loss function component can contribute to the model performance for different tasks under various settings; 
\textit{(ii)} the multi-grained pooling and unpooling process can do improve the model performance compared with different \textit{flat} advanced GNNs. 
% \CL{(need to briefly present the results of this ablation study here)}
% \JP{I don't see whether any revision has been made to satisfy this reviewer's complain. If yes, add sentences to explain what changes and where they are.}
}

\smallskip\noindent
\textbf{7.} ``It would be better if the authors could go through the paper carefully and improve the writing.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks. Following your suggestion, we have carefully gone through the writing and fixed a few typos.
}

\smallskip\noindent
\textbf{Comments from Reviewer 2}

\smallskip\noindent
\textbf{1.} ``The claim “Existing studies solve either the node-wise task or the graph-wise task independently while they are inherently correlated” is not entirely true. For example, Graph U-Net is used for both graph classification and node classification tasks. It is important to clarify the difference.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for pointing out this issue. Following your comments,
we have adjusted the claim in Abstract and carefully discussed the differences between G-U-Net and AdamGNN in the last paragraph of Section~2. 
% 
%\CL{(for each of below points, we should not only describe what G-U-Net does, but emphasize how our AdamGNN differs/improves from G-U-Net?)}
Specifically, (1) the Top-\textit{k} selection strategy of G-U-Net introduces a new hyper-parameter ($k$) and may lose important node features or graph structure by simply dropping non-selected nodes (on the contrary, AdamGNN designs an adaptive pooling operator that can automatically decide the super node number and main a proper super graph size, see Section 4.3, Visualisation of different granularity levels, Figure~5); 
% \CL{(briefly describe what is the hyperparameter and how does it bring info loss?)}
(2) G-U-Net generates the super graph only with $k$ selected super nodes, which ruins multi-grained semantics of the original graph (on the contrary, AdqmGNN's adaptive pooling operator maintains useful node features and multi-grained semantics);
(3) G-U-Net does not support mini-batch because it needs to compute scores of all nodes in one big batch to select super nodes (on the contrary, AdamGNN supports efficient mini-batch pooling and unpooling operators).
Besides, AdamGNN also achieves a mutual optimisation between node- and graph-wise tasks and provides model explanation via multi-grained semantics. 
Therefore, we believe AdamGNN's framework is more general, effective and scalable than G-U-Net. 
}

\smallskip\noindent
\textbf{2.} ``The overall structure of the proposed model is very similar to Graph U-Net, which also employs graph pooling and graph unpooling. Again, it is important to clarify the difference and demonstrate the contribution, otherwise, the technical contribution seems to be limited. This is my main concern for this work. In addition, the top-k selection strategy also follows Graph U-Net.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your critical comment, and we agree that both G-U-Net and AdamGNN adopt pooling and unpooling operators. 
But we kindly urge reviewers notice that G-U-Net and AdamGNN have different designs and G-U-Net does not support novel aggregation mechanism of AdamGNN (as shown in Section 4.3, Comparing aggregation mechanism).
%
Specifically, first, the differences between G-U-Net and AdamGNN are addressed in the last paragraph in Section 2 and summarised in the previous response. 
% 
Second, it should be noted that AdamGNN does not use the top-$k$ selection strategy, which is one of the significant differences from G-U-Net.
The top-$k$ selection strategy of G-U-Net introduces an additional hyper-parameter ($k$), which is significantly crucial for the final performance, thus reducing the convenience in applications with different scale graphs (the second paragraph of Section 1). 
The top-$k$ selection strategy restricts G-U-Net to the mini-batch pipeline because it needs to compute scores of all nodes in one big batch to compose super nodes. 
Moreover, it is easy to lose important node features and graph structure by only utilising $k$-selected super nodes and simply dropping non-selected nodes, as shown in Figure~1.
% 
On the contrary, the adaptive pooling and unpooling operators of AdamGNN do not introduce any hyper-parameters as described in Section~3.2 and Section~3.3. 
AdamGNN enhances node representations with multi-grained semantics, but G-U-Net only involves selected super nodes in the super graph and drop non-selected nodes, breaking the graph structure's multi-grained semantics. 
Moreover, AdamGNN has better scalability than G-U-Net, since AdamGNN is designed as a local network algorithm that enables AdamGNN to be friendly to distributed computing settings. 
% 
At last, we express our understanding that it was easy to misunderstand that AdamGNN also utilises the Top-$k$ selection strategy, because we used ($K \& k$) to present the granularity levels in the previous version.
We revised them as $T \& t$ and polished Section 3 to avoid misunderstanding. 
}

\smallskip\noindent
\textbf{3.} ``Another question is about “Maintaining super graph connectivity”. I think it is the same strategy as Diffpool and Structpool. Is there any difference I did not notice? In addition, such a strategy will lead to a denser graph in level k-1. Will this be a problem?''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for noticing this, we have revised the third paragraph of Section~4.3 to clarify and address your concern.
% 
The graph pooling models, DiffPool, G-U-Net, SagPool, StructPool, ASAP and AdamGNN utilise a similar strategy described in ``Maintaining super graph connectivity''. 
The \textit{dense} issue of DiffPool and StructPool is mainly caused by the dense assignment matrix (used for pooling) [4]. 
AdamGNN is designed as a local network algorithm (Section 3.6, Model Scalability) that has no one big and dense assignment matrix to avoid the dense issue. 
%\CL{(why? be concrete to explain why our local algorithm will not have dense assignment matrix -- this is the key to answer this question)}
That said, for DiffPool and StructPool, is they want to pool a graph $\mathcal{G}_k$ with $n$ nodes to a super graph $\mathcal{G}_{k+1}$ with $m$ nodes, they need a $n \times m$ assignment matrix.
On the contrary, AdamGNN only need to check each node with their local neighbouring nodes to decide who is going to be a super node and the assignment matrix with size of $n \times 1$, and the assignment matrix can be easily divided into up to $n$ mini-bitch if needed for distributed computing. 
% 
In addition, about the pooling process from level $k-1$ to level $k$. 
The dense problem that the reviewer worried about is too many nodes are summarised as a few super nodes then all relations from those nodes are generated to a few super nodes. 
Such an issue may happen with top-$k$ pooling which strictly follows a predefined pooling ratio ($k$) for each level and after multiple pooling operations, it will generate a very dense super graph.
On the contrary, AdamGNN designs an adaptive pooling operator which does not strictly follow a fixed pooling ratio and will stop pooling super nodes at a certain level.
For example, as shown in Figure~5, AdamGNN can adaptively pool nodes as super nodes, and maintain the graph size at a proper level (Section~4.3 - Visualisation of different granularity levels).
Therefore, it will not always reduce the graph size to form a much denser graph (in terms of edge numbers) as other graph pooling methods using the Top-$k$ selection strategy. 
So, the ``Maintaining super graph connectivity'' part should not be a significant problem for AdamGNN.
% \CL{(after reading this paragraph, I still cannot capture the idea about why our method avoids generating dense super graphs -- this is the concern of this reviewer)}
}

\smallskip\noindent
\textbf{4.} ``The graph unpooling is unclear to me. Could you provide an example to explain? It is not clear how to map the nodes in level k-1 to level k.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for highlighting this unclear part. Following your suggestions, we have revised Figure~2-(b) and the second paragraph of Section 3.3 to explain the unpooling process. 
% 
As shown in Figure~2-(b), graph pooling and graph unpooling are two inverse processes that are realised by $\mathbf{H}_{t-1}\mathbf{S}_{t}$ and $\mathbf{H}_{t}\mathbf{S}^{\mathrm{T}}_{t}$. 
That said, the assignment matrix $\mathbf{S}_t$ records how nodes in $\mathcal{G}_{t-1}$ are pooled as super nodes in $\mathcal{G}_{t}$.
Then, we can use $\mathbf{S}_{t}$ for pooling and unpooling. 
}

\smallskip\noindent
\textbf{5.} ``For experimental studies, how different methods are compared? For example, different pooling methods share a similar pipeline: graph encoder+ pooling+ classifier. In their papers, the encoders can be very different. When conducting a comparison, it is important to use the same encoder and classifier. Similarly, for node classification tasks, the settings should also be fair enough.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your comments. We agree that the fairness of experimental comparison is essential, and we need to clarify them. 
We have added more detailed descriptions in the ``Model configuration'' part of Section~4.1, and we have uploaded our code, including the implementations of competing methods on Github~\footnote{\url{https://github.com/zhiqiangzhongddu/AdamGNN}} for reproducing our experiments. 
% 
Specifically, as described in Section~4.1 (Model configuration), we adopt GCN as the default GNN encoder for all graph pooling models, if needed. 
And they follow the same pipeline as graph encoder + pooling + classifier. 
}


\smallskip\noindent
\textbf{6.} ``How is the time cost comparison for node classification tasks?''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for pointing out this important issue.
We added a paragraph at the end of Section~3.6 to analyse the scalability of AdamGNN and added the execution time of AdamGNN for the node classification task in Table~11.
% 
Specifically, we added the average one epoch running time for node classification and graph classification tasks in Table 11 and Table 12. 
For the graph classification task, the graph size is smaller, and AdamGNN does not need the \textit{dense} assignment matrix and supports mini-batch computing; hence it strikes a balance between performance improvement and maintaining proper time efficiency. 
We find that AdamGNN requires more training time for the node classification tasks. 
It is because of the computation cost of $\alpha_{ij}$ and $\beta$. 
Such a shortcoming is a common issue of attention-enhanced models [5].
But we tried to resolve this issue by implementing the node classification pipeline with a multi-GPU computing framework [6].
As shown in Table~11, such an issue can be significantly alleviated by mini-batch and multi-GPUs computing framework due to the local network algorithm design of AdamGNN. 
And, given the effectiveness and versatility of AdamGNN, we argue it is still a promising model for advanced graph representation learning tasks. 
}

\smallskip\noindent
\textbf{7.} ``Typos: Line 17- “Experiments conducted on 13 real-world graphs”- graphs to graph datasets.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks. Following your suggestion, we have carefully gone through the writing and fixed a few typos.
}

\smallskip\noindent
\textbf{Comments from Reviewer 3}

\smallskip\noindent
\textbf{1.} ``On one hand, the proposed method is not evaluated on several newly proposed benchmarks, such as the OGB. The reviewer is also concerned about whether the proposed method scales well to large graphs, as the largest graph this paper uses is Pubmed, which only has 19,717 nodes.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for your suggestion. Following your suggestions, we have added a new OGB dataset, i.e., Ogbn-arxiv [7], and have updated the experimental results with competing models in Table~4. We discussed the updated results in the first paragraph of Section 4.2. 
Briefly, AdamGNN has competitive performance on Ogbn-arxiv compared with a set of state-of-the-art methods. 
% \CL{(need to briefly summarize the results here)}
% 
% \JP{Clearly explain where are the new results!}
}

\smallskip\noindent
\textbf{2.} ``On the other hand, some baseline results reported in Table 4 do not exactly match their originally reported results, even though this paper claims that it uses identical experimental setup for semi-supervised node classification. For example, GCN achieves 81.5 (accuracy on Cora, and GAT achieves 83.0; accuracy, while this paper reports 80.41 and 81.40, respectively).''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the detailed comments. We agree our descriptions of ``Evaluation settings'' were not precise enough.
We have revised the ``Evaluation settings'' of Section~4.1 to specify that we ``randomly assign 20 labelled nodes for each class for training, and 50 and 1000 nodes for validation and testing, respectively.'' 
% 
Particularly, the GCN paper [3] adopts a fixed split that means they fixed one group of train/valid/test splits for experiments.
We follow their approach to randomly split train/valid/test datasets for semi-supervised node classification experiments.
That said, randomly assigning 20 labelled nodes for each class for training, and 500 and 1000
nodes for validation and testing, respectively.
And since other datasets do not have available fixed splits, we randomly generated $10$ splits for experiments instead of one fixed split.
Therefore, the experimental results might slightly vary. 
% 
Moreover, it should be noted that AdamGNN endows the \textit{flat} GNN with multi-grained semantics. Hence, it is theoretically helpful for any \textit{flat} GNN encoder, as shown in the ablation study of Section~4.3 (Ablation study of different primary GNN encoders, Table~10). 
}

\smallskip\noindent
\textbf{3.} ``Besides,  this paper does not include several newly published models as baselines, such as GCNII [1] and GRAND [2]. These models capture the global information via propagating more steps. For example, GCNII could propagate 64 times for Cora, which is far more than the diameter of Cora, and is sufficient to aggregate the global information.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for the useful suggestions. Following your comments, we have added the experimental results by further comparing AdamGNN to GCNII and GRAND in Section~4 (Tables~4, 5, 10). We discussed the results (Section~2) and compared them with AdamGNN (Table~1). 
% 
Moreover, it should be noted that AdamGNN endows the \textit{flat} GNN with multi-grained semantics. Hence, it is theoretically helpful for any \textit{flat} GNN encoder, as shown in the ablation study of Section~4.3 (Ablation study of different primary GNN encoders, Table~10). 
GCNII can stack lots of layers to capture long-range information; however, it still follows a \textit{flat} message-passing mechanism hence naturally ignoring the multi-grained semantics.
AdamGNN could further alleviate this problem for better performance. 
% \JP{Clearly explain we have referred to these new models, discussed them, and compared them, and point to where are the new materials!}
}

\smallskip\noindent
\textbf{4.} ``The fitness score (Eq.~2), the importance score $\alpha$ (Eq. 5), and the flyback aggregation score $\beta$ (Eq.~7) are implemented as attention score. Will this cause heavy computational complexity on large graphs?''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for pointing this important issue. We agree that such a shortcoming is a common issue of attention-enhanced models [5].
We added a paragraph at the end of Section~3.6 to analyse the scalability of AdamGNN. We added the execution time of AdamGNN for the node classification task in Table 11, which exhibits the computational complexity that can be alleviated by mini-batch and multi-GPU computing. 
Particularly, we presented the average one epoch running time for node classification and graph classification tasks in Table~11 and Table~12. 
For the graph classification task, the graph size is smaller, and AdamGNN does not need the \textit{dense} assignment matrix and supports mini-batch computing; hence it strikes a balance between performance improvement and maintaining proper time efficiency. 
We find that AdamGNN requires more training time for the node classification task. 
It is because of the computation cost of $\alpha_{ij}$ and $\beta$. 
Such a shortcoming is a common issue of attention-enhanced models [5].
As shown in Table~11, such an issue can be significantly alleviated by mini-batch and multi-GPUs computing framework [6] due to the local network algorithm design of AdamGNN. 
The promising effectiveness and versatility of AdamGNN supports its usefulness for graph representation learning. 
}

\smallskip\noindent
\textbf{5.} ``What's the functionality of the LeakyReLU inside the score calculation in Eq.2, if the softmax function provides the non-linearity?''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for noticing it. We have revised the third paragraph of Section~3.2 to clarify it. 
% 
The closeness scores calculated by Eq.~2 works as weights of $\mathbf{S}_t$ to generate the super graph of granularity level $t$ and learn the semantic information of granularity level $t$. 
So, the results of Eq.~2 will be the component of the final learned representations.
We add $\mathrm{LeakyReLU}$ in Eq.~2 to avoid the vanishing gradient problem [8] during the model training process. 
}

\smallskip\noindent
\textbf{6.} ``It seems that the granularity is strongly connected with the hyper-parameter $\lambda$ in the definition of the ego-network. While this paper argues that the hyper-parameter $k$ is importance for the Top-$k$ selection in Graph U-Nets, will the proposed method be affected by $\lambda$?'

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the insightful suggestion. 
We agree it is very interesting to investigate the influence of $\lambda$. 
We have added an ablation study to investigate the influence of $\lambda$ in Section~4.2 (Ablation study of Ego-network size ($\lambda$), Figure~3) on three different downstream tasks. 
% 
The experimental results indicate that $\lambda$ has no significant influence on the performance. 
Because in the super node determination process, each node may belong to various ego-networks since they may play different roles in different groups. 
Larger $\lambda$ leads to larger ego-networks while allowing multiple ego-networks to present the multi-grained semantics of each node.
Therefore, the performance of AdamGNN will not be significantly influenced by $\lambda$. 
% \JP{Make it explicit what are newly added materials, and where are they.}
}

\vspace{10mm}\noindent
{\bf References:}

\noindent
[1] Chen et al. Simple and deep graph convolutional networks. ICML, 2020.

\noindent
[2] Feng et al. Graph Random Neural Network for Semi-Supervised Learning on Graphs. NeurIPS, 2020. 

\noindent
[3] Kipf et al. Semi-supervised classification with graph convolutional networks. ICLR 2017. 

\noindent
[4] Raswani et al. ASAP: adaptive structure aware pooling for learning hierarchical graph representations. AAAI, 2020

\noindent
[5] Vaswani et al. Attention is all you need. NIPS, 2017

\noindent
[6] Kaler et al. Accelerating Training and Inference of Graph Neural Networks with Fast Sampling and Pipelining. arxiv, 2021

\noindent
[7] Hu et al. Open graph benchmark: Datasets for machine learning on graphs, NeurIPS, 2020. 

\noindent
[8] Sepp Hochreiter. The Vanishing Gradient Problem During Learning Recurrent Neural Nets and Problem Solutions. International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems, 1998. 


==> pages/response_letter_2.tex <==
\onecolumn
\section{Response Letter}
Dear Reviewers and Editors,

\smallskip
Thank you for giving us the opportunity to submit a revised draft of our manuscript titled ``Multi-grained Semantics-aware Graph Neural Networks” to IEEE Transactions on Knowledge and Data Engineering. 
We appreciate the time and efforts you and the reviewers have dedicated to providing your valuable feedback on our manuscript. 
We are grateful to the reviewers for their insightful comments and suggestions on our paper which helped us find shortcomings of our manuscript in terms of model design and paper writing. 
We have been able to incorporate changes to reflect most of the suggestions provided by the reviewers. 
Below is a point-by-point response to the reviewers’ comments and concerns.


\smallskip\noindent
\textbf{Comments from Reviewer 1}

\smallskip\noindent
\textbf{1.} ``Explains that AdamGNN is not sensitive to the granularity (controlled by $\lambda$) when compared with Graph U-Nets (controlled by k).''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for this insightful suggestion. 
We agree it is very important to investigate the influence of $\lambda$. 
We have added an ablation study to investigate the influence of $\lambda$ in Section~\ref{subsec:experimental_evaluation_and_ablation_study} (Ablation study of Ego-network size ($\lambda$), Figure~\ref{fig:different_lambda}) on three different downstream tasks. 
% 
The experimental results indicate that $\lambda$ has no significant influence on the task performance. 
Because in the super node determination process, nodes may belong to various ego-networks since they may play different roles in different groups. 
Larger $\lambda$ leads to larger ego-networks while allowing multiple ego-networks to present the multi-grained semantics of each node.
Therefore, the performance of AdamGNN will not be significantly influenced by $\lambda$. 
}

\smallskip\noindent
\textbf{2.} ``Make a thorough investment in relevant literature. For example, graph cross network also adopt a similar strategy (up-/down-sampling).''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for noticing this. 
We revised Section~\ref{sec:introduction} and Section~\ref{sec:related_work} to add more relevant work that adopt a similar strategy. We also carefully discussed the difference between AdamGNN and closely relevant models in the last paragraph of Section~\ref{sec:related_work}. 
Specifically, (1) the Top-\textit{k} selection strategy of \textsc{g-U-Net} and GXN introduces a new hyper-parameter ($k$) and may lose important node features or graph structure by simply dropping non-selected nodes (on the contrary, AdamGNN designs an adaptive pooling operator that can automatically decide the super node number and maintain a proper super graph size, see Section~\ref{subsec:more_model_analysis}, Visualisation of different granularity levels, Figure~\ref{fig:different_levels}); 
(2) Both \textsc{g-U-Net} and GXN generate the super graph only with $k$ selected super nodes, which may lose multi-grained semantics of the original graph (on the contrary, AdqmGNN's adaptive pooling operator maintains useful node features and multi-grained semantics);
(3) \textsc{g-U-Net} does not support mini-batch because it needs to compute scores of all nodes in one big batch to select super nodes (on the contrary, AdamGNN supports efficient mini-batch pooling and unpooling operators);
(4) GXN requires the sampling of positive and negative node sets, which introduces additional operations. The random sampling also brings unmanageable uncertainty on performance [1] (on the contrary, AdamGNN achieves adaptive pooling process without additional operations).
(5) Besides, AdamGNN also achieves a mutual optimisation between node- and graph-wise tasks, and provides model explanation via multi-grained semantics. 
Therefore, we believe AdamGNN's framework is more general, effective, and scalable than \textsc{g-U-Net} and GXN. 
% 
Moreover, to have convincing experimental evaluation, we have updated the results of node classification, link prediction and graph classification results by adding GXN in Table~\ref{table:nc_results}, Table~\ref{table:lp_results} and Table~\ref{table:gc_results}, respectively. 
From the reported results, we can find that AdamGNN outperforms GXN in terms of three tasks. 
Note that, during the experimental reproduction, we found that our reproduced GXN results were less good than the results reported in the official paper of GXN. 
And taking the issues on GXN's official GitHub page\footnote{\url{https://github.com/limaosen0/GXN}} into account, we think there exist unfair settings (for instance, there are incorrect testing data split and loss computation errors) in GXN's experiments, and we are not able to obtain similar performance as reported in GXN's paper. 
}

\smallskip\noindent
\textbf{Comments from Reviewer 2}

\smallskip\noindent
\textbf{1.} ``As per the response from the authors, it is still unclear what ``sematic-aware'' means. Especially, the provided example does not motivate the necessity of introducing multi-grained representations.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for pointing out this issue. 
The multi-grained semantics is motivated by two aspects. 
First, following the example academic collaboration network that we discussed in Section~\ref{sec:introduction}, there exists the semantics at different granularity levels in real-world networks. 
For instance, the raw academic collaboration network presents the micro semantics (e.g., co-authorship) between authors, but it cannot present macro semantics (e.g., belonging to different research institutes). 
Intuitively, one person's property can be defined not only in terms of the person itself, but it is also helpful to refer to the group to which the person belongs to. 
Second, as we presented in Section~\ref{sec:introduction} and Section~\ref{sec:related_work}, graph pooling operations have been proven to be useful to mine graph representations in a multi-grained manner. 
Therefore, we argue it could be a promising and effective manner to learn node representations that contain multi-grained semantics. 
Moreover, AdamGNN also achieves a mutual optimisation between node- and graph-wise tasks and provides model explanation via multi-grained semantics.
}

\smallskip\noindent
\textbf{2.} ``2. It is still not clear why we need both non-linear and linear relations for measuring the closeness score. Also, why the first part is regarded as non-linear while the second part is regarded as linear? There is sigmoid in the second part, which is also non-linear.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your insightful comment, and we have revised Section~\ref{sec:proposed_approach} to better motivate the design of Eq.~\ref{eq:fiscore}.
Specifically, Eq.~\ref{eq:fiscore} is designed to compute the similarity between nodes and the ego. 
In order to achieve such an objective, we propose to evaluate the linear and non-linear closeness between them. 
The idea of combining different operations to get more comprehensive information has been confirmed in recently published papers.
For instance, Corso et al. [2] design different scalers (linear and non-linear) to combine different messages from neighbours. 
% 
In addition, the $\mathrm{Sigmoid}$ of $f^{\it lin}_{\phi}(v_{i}, v_{j})$ only re-scales the results into a proper range (i.e., (0, 1)), it does not change the way of defining the similarity of Eq.~\ref{eq:fiscore}. 
Therefore, we argue the similarity given by Eq.~\ref{eq:fiscore} is computed by $\mathbf{H}^{\mathrm{T}}[j] \cdot \mathbf{H}[i]$. 
}

\smallskip\noindent
\textbf{3.} ``It would be better if the authors also include the results based on the standard-setting as in GCN to make a more fair comparison.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for this concrete suggestion. 
Following your suggestions, we update our data splitting settings of \textit{semi-supervised node classification} (Semi-NC) as shown in Section~\ref{subsec:experimental_setup} (Evaluation settings). 
For Cora, Citeseer and Pubmed datasets with available fixed splits, we use the fixed splits given by [3]. 
For other datasets without available fixed splits, we randomly assign training, validation, and testing node sets similarly to [3].
% 
The related experimental results are updated accordingly, as shown in Table~\ref{table:nc_results} and Table~\ref{table:ablation_analysis_primary_encoder}. 
% 
The results of Table~\ref{table:nc_results} indicate that AdamGNN can outperform most competing methods with up to $10.47\%$ and $5.39\%$ improvements on semi-supervised and supervised settings, respectively.
Morevoer, from Table~\ref{table:ablation_analysis_primary_encoder}, we can find that AdamGNN with advanced GNN encoders can achieve better performance. 
That said, advanced GNN encoders can still benefit from the multi-grained semantics of AdamGNN. 
So, we think it is a promising and practical way to boost GNN models' performance with the framework of AdamGNN. 
}

\smallskip\noindent
\textbf{Comments from Reviewer 3}

\smallskip\noindent
\textbf{1.} ``In graph pooling, the value of $k$ can be very important. How do you select the value of $k$ in the experimental studies for other comparing methods? The proposed AdamGNN can automatically decide the supernode number but other techniques, such as Graph Unet, Diffpool, Structpool, need a proper $k$ to obtain good performance. Also, if we apply the $k$ value that obtained by AdamGNN to other methods, will they also have better performance? It would be very interesting to see such studies.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your critical comment. We agree that the value of $k$ can be very important.
In terms of the settings of $k$ value in the experimental studies for competing methods, as described in Section~\ref{subsec:experimental_setup} Model configuration, we employ the same settings of each competing model shown in each paper's official implementation.
The detailed implementation refers to our published code. 
% 
With respect to the possibility of assigning the adaptively learned value of $k$ for other pooling methods,
since the existing implementations of \textsc{g-U-Net}, Diffpool and Structpool use one default $k$ value for all layers, we are not able to assign different $k$ values to different levels with the published code. 
% 
Moreover, we argue that the significant difference between AdamGNN's pooling operation and graph pooling models is not only the number of selected super nodes at each level but also the approach to choosing super nodes. 
}

\vspace{10mm}\noindent
{\bf References:}

\noindent
[1] Yang et al. Understanding Negative Sampling in Graph Representation Learning. KDD, 2020.

\noindent
[2] Corso et al. Principal Neighbourhood Aggregation for Graph Nets. NeurIPS, 2020.

\noindent
[3] Kipf et al. Semi-supervised classification with graph convolutional networks. ICLR, 2017.

